Verilog-to-PyG -- A Framework for Graph Learning and Augmentation on RTL Designs

The complexity of modern hardware designs necessitates advanced methodologies for optimizing and analyzing modern digital systems. In recent times, machine learning (ML) methodologies have emerged as potent instruments for assessing design quality-of-results at the Register-Transfer Level (RTL) or Boolean level, aiming to expedite design exploration of advanced RTL configurations. In this presentation, we introduce an innovative open-source framework that translates RTL designs into graph representation foundations, which can be seamlessly integrated with the PyTorch Geometric graph learning platform. Furthermore, the Verilog-to-PyG (V2PYG) framework is compatible with the open-source Electronic Design Automation (EDA) toolchain OpenROAD, facilitating the collection of labeled datasets in an utterly open-source manner. Additionally, we will present novel RTL data augmentation methods (incorporated in our framework) that enable functional equivalent design augmentation for the construction of an extensive graph-based RTL design database. Lastly, we will showcase several using cases of V2PYG with detailed scripting examples. V2PYG can be found at \url{https://yu-maryland.github.io/Verilog-to-PyG/}.

==> compiler-table.tex <==
\begin{table*}[h]
\scriptsize
    \centering
\begin{tabular}{|p{5em}|p{12em}|p{41em}|}

     \midrule
     Classes & Modular Programs & Description\\
     \midrule
     
     \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\\ \\ \\ ~~Low-level \\ ~~~modeling\end{tabular}} & Laser source \& profiles & The source emitting coherent laser beam with specific wavelength and profile, e.g., Gaussian beam, Bessel beam, etc. \\
     
     \cmidrule(r){2-3}
     
     & Diffraction approximation & High-performance tensor implementations of numerical diffraction approximations, including \textbf{Rayleigh-Sommerfeld} (Equation \ref{equ:sommerfeld}), \textbf{Fresnel} (Equation \ref{equ:fresnel}), and \textbf{Fraunhofer} (Equation \ref{equ:fraunhofer}).  \\
     \cmidrule(r){2-3}
     
     & Optical/photon detector & An photon detector to capture the light intensity and convert the analog intensity information to the digital computer-processable information. \\
     \midrule
 
     \multirow{4}{*}{ \begin{tabular}[c]{@{}c@{}} \\ \\ \\ Model-level\\ APIs\end{tabular}} & \texttt{lr.laser} & Define the laser source for the system, including laser wavelenghth and it profile. \\
     \cmidrule(r){2-3}
    & \vspace{1mm}\texttt{lr.layers} & Includes modules of different types of diffractive modeling, e.g., hardware-specific layer module \texttt{lr.layers.diffractlayer} and general diffractive layer \texttt{lr.layers.diffractlayer\_raw}, that can be configured with various approximation methods, distance, diffraction unit size, etc. \\
    \cmidrule(r){2-3}
    & \texttt{lr.layers.detector} & Define detector designs for various computer vision ML tasks, e.g., classification detector with coordinate information and the size of the detector regions. \\
    \cmidrule(r){2-3}
    & \texttt{lr.models} & Sequential container to customize DONN system by stacking diffractive layer and detector modules.\\
     \midrule
     
     
     \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \\  ~~~Training \end{tabular}} &  \vspace{0.2mm}\texttt{lr.train.utils} & Training utility modules including data handling (e.g., \texttt{utils.data\_to\_cplex}), complex-valued regularization, loss function, optimizer, etc.\\
     \cmidrule(r){2-3}
         & \texttt{lr.layers.to(device)} & Enable CPU and GPU accelerations for accelerating diffraction emulation and DONNs training.  \\
        % \cmidrule(r){2-3}
        % & \texttt{lr.traioptimizer} & Visualization of emulated propagation process through the system. \\
        \midrule
    \multirow{2}{*}{\begin{tabular}[|c|]{@{}c@{}}  Hardware \\ deployment\end{tabular}}  & \texttt{lr.layers.weight\_dump} & Quantize the phase weights in the trained model w.r.t the hardware (e.g., SLMs) specifications. \\
    \cmidrule(r){2-3}
    
    &\texttt{lr.model.to\_system} & Hardware deployments modules, e.g., \texttt{lr.model.to\_slm()}, \texttt{lr.model.to\_3d\_render()}, etc. \\
     \midrule
\end{tabular}
  \vspace{-3mm}
      \caption{Overview of the LightRidge programming modules and sample front-end language examples. Note that we use \texttt{lr} to represent our package \texttt{lightridge}.}
    \label{tab:language}
\end{table*}


\iffalse
\begin{table*}[]
\small
    \centering
    \begin{tabularx}{\linewidth}{  
    | >{\raggedright\arraybackslash}p{5em} 
    | >{\raggedright\arraybackslash}p{16em}
    | >{\raggedright\arraybackslash}X |}
    \hline
         class & Modular Prog. & Description\\
         \hline
         \multirow{3}{*}{\begin{tabular}[|c|]{@{}c@{}}lower-level \\ module\end{tabular}} & \texttt{lr.laser} & Define the laser source for the system, including laser wavelenghth and it profile, e.g., Gaussian beam, Bessel beam, etc. \\
         \cmidrule(r){2-3}
         & \texttt{\texttt{lr.layers.DiffractLayer}} & Define the detailed diffraction information in the system, including the size information of diffractive layers, the diffraction approximation methods, the diffraction distance between layers, etc. \\
         \cmidrule(r){2-3}
         & \texttt{lr.layers.Detector} & Define the pre-defined detector regions for each class on the detector plane, including the coordinate information and the size of the detector region for each class. \\
         \hline
         DONN Model & \texttt{Class Model(): ...} & Customize the DONN system by stacking defined diffractive layers and detector plane in arbitrary ways.\\
         \hline
         \multirow{3}{*}{high-level module} & \texttt{train(model, device, ...)} & Call the training function where dataset, optimizer, loss function, learning rate, etc are defined.\\
         \hline
         & \texttt{model.phase\_view()} & Visualization of phase modulation in each diffractive layer. \\
         \hline
         & \texttt{model.prop\_view()} & Visualization of emulated propagation process through the system. \\
         \hline
         Hardware deployment & \texttt{model.to\_slm() model.to\_3d\_render()} & Provide interface with hardware backends. \\
         \hline
         
    \end{tabularx}
    \caption{{Illustration for the modular program block in the compiler. We first import \texttt{LightRidge} as \texttt{lr}.}
    \label{tab:language}}
\end{table*}
\fi

==> isca2022-latex-template/01-intro.tex <==
\section{Introduction}

The increasing complexity of electronic systems has driven significant advancements in hardware design. Modern hardware designs encompass a wide range of components, from Register Transfer Level (RTL) descriptions to logic circuits. As the complexity of these designs grows, the need for effective optimization and analysis techniques becomes more critical. One promising approach to addressing these challenges is through the application of graph learning techniques.

Graph learning has emerged as a powerful method for understanding complex relationships in various domains, including social networks, biological systems, and natural language processing. In the context of hardware design, graph learning can be employed to model and analyze the intricate connections among design components, such as gates, wires, and registers, to optimize design performance and effectively analyze design characteristics.

Recently, machine learning (ML) has been applied to computer systems and electronic design automation (EDA) tasks~\cite{wu2022survey} as an alternative to conventional design solutions. Circuit netlists or Boolean networks (BNs) can be easily represented as graphs, making graph neural networks (GNNs) a natural fit for classifying sub-circuit functionality from gate-level netlists~\cite{alrahis2021gnn}, analyzing the impacts of circuit rewriting~\cite{zhao2022graph}, predicting arithmetic block boundaries~\cite{he2021graph}, and improving the fidelity of early-stage design exploration \cite{ustun2020accurate}.

However, when applying graph learning to RTL designs, there is a lack of support for dataset preparation, particularly in graph representations of RTL designs. Two primary challenges exist: 1) The absence of comprehensive infrastructure support that connects RTL designs with graph representations, facilitates graph dataset construction, and seamlessly integrates with existing graph learning frameworks such as PyTorch Geometric (PyG) \cite{fey2019fast}. 2) The limited availability of design variations for training and potential search spaces for RTL foundation models, necessitating the development of effective RTL design augmentation techniques. To address these challenges, we introduce an open-source infrastructure that establishes compatibility with PyG \cite{fey2019fast} and enhances the variety of RTL design samples through functionally equivalent RTL augmentations.

{\color{red} need to expand the intro, particularly on the challenges of lacking infrastructures; }



==> isca2022-latex-template/03-v2pygFrame.tex <==
\section{V2PyG Framework}
\label{sec:framework}

\subsection{Features for ML4EDA}

{\color{red} high-level summary; can check the ISCA slides kind of link to why Graph representations are important?}

\subsection{Verilog to Graph Representation}
\label{subsec:embedding}

V2PYG currently performs Verilog to graph representation at the foundation of Boolean representations, including technology dependent (technology mapped) and technology independent representations (Boolean networks such as And-Inv-Graphs). V2PYG parses Verilog designs using Yosys front-end and performs downstream design flow via OpenROAD. In this abstract paper, we focus on discussing how sequential design can be represented as combinational design is a special case. First, transform the sequential design into an equivalent design using Boolean network datastructure (e.g., AIGs), or technology dependent networks (exact topology of mapped netlist). Next, model flip-flops as pseudo-primary inputs (PPIs) and pseudo-primary outputs (PPOs), connecting them through the AIG network to capture state transitions and dependencies between flip-flops and combinational logic. Data labels will be generated via OpenROAD \cite{ajayi2019toward} downstream flow. As a result, the sequential design will be represented in semi-complete multi-DAGs. Our on-going effort aims to integrate MLIR CIRCT \cite{circt} into the pipeline to process multi-fidelity graph representations (DFGs w Boolean networks). 

\begin{figure}[!htb]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/sample/b11_sample.pdf}
        \caption{b11}
        \label{fig:sample_b11}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/sample/b12_sample.pdf}
        \caption{b12}
        \label{fig:sample_b12}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/sample/c2670_sample.pdf}
        \caption{c2670}
        \label{fig:sample_c2670}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/sample/c5315_sample.pdf}
        \caption{c5315}
        \label{fig:sample_c5315}
    \end{subfigure}
    
    \caption{The optimization quality distribution with 6000 samples of purely random sampling and priority guided sampling. %The guided sampling can result in more samples with better AIG optimization.
    }
    \label{fig:sample}
\end{figure}


\subsection{Combinational Augmentation}



\begin{algorithm}
\caption{Boolean manipulation sampling on AIGs}   
%\begin{algorithmic} %\begin{algorithmic}[1]
%\vspace{-2mm}
\footnotesize
\label{alg:orch}
 
   \SetKwInOut{KwIn}{Input}
     \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{~$G(V,E) \leftarrow$ Boolean Networks/Circuits in AIG} 
    \KwIn{Per node manipulation decision $D$, $|D| = |V|$}
    \tcp{$D$ saved as an Array $D$, e.g., $D[1] = 0$ indicates the optimization for node $1$ is $0(1)$, i.e., \texttt{rw}(\texttt{rs}).}
    \KwOut{~Post-optimized AIG $G(V,E)$}
 \For{$v \in V$ in topological order}{
 %\tcp{New order}
  \uIf{v \text{is transformable w.r.t} $D[v]$}{
        $ G(V,E) \xleftarrow{D[v]} G(V,E)$
        continue
     \tcp*[f]{check the transformability with the assigned optimization}
         }

  \Else{
    continue 
  }
  Update $G(V,E) \leftarrow$ \texttt{Dec\_GraphUpdateNetwork}, and exclude $v$ and transformed nodes from $V$
  }
%  \end{algorithmic}
\end{algorithm}

{\color{red} combinational augmentation is basically just variations of AIG random synthesis. 1) first talk about each synthesis function. 2) show the example and then random sampling via algorithm1 ; 3) show the AIG example Fig 2 and discuss the QoR variations (sufficient for ML? - a discussion)}
The combinational augmentation of RTL designs can be achieved through V2PYG by applying transformations that maintain combinational equivalence. Specifically, V2PYG incorporates data flow augmentation using polynomial manipulations, fine-grained Boolean algebra manipulation (at least at the individual Boolean node level), and graph isomorphism augmentation. These augmentation techniques enable the generation of a nearly unlimited number of functionally equivalent designs at the Boolean level.

\subsection{Sequential Augmentation} -- V2PYG currently supports sequential augmentation by adjusting the Data Flow Graph (DFG) level scheduling and fine-grained retiming (per Boolean node), providing significant design variations while preserving sequential equivalence. It is important to note that combinational augmentation is orthogonal to sequential augmentation.

{\color{red} need to expand the sequential one; retiming?}



==> sec-compiler-old.tex <==
\section{LightRidge Compiler}\label{sec:overview}

%{\color{red} paragraph will be expanded to subsections later.}

\begin{figure}[t]
  \centering
  \includegraphics[width=1 \linewidth]{isca2022-latex-template/figs/new_figure/compiler_system_overview_new.pdf}
  \caption{\color{blue}Overview of LightRidge compilation stack, including design, emulation, training, and deployment.}
  \label{figs:overview}
\end{figure}


{In this section, we describe the programming modules implemented in LightRidge. Our framework (Figure \ref{figs:overview}) aims to simplify and accelerate the process of design, exploration and deployment of the DONNs, such that it consists of \textbf{a)} versatile programming modules for user-defined optical systems, \textbf{b)} optical laser modules, \textbf{c)} physics modeling of diffraction, \textbf{d)} system measurement modeling under optical meaning, \textbf{e)} DONN architecture construction and physics-aware training, and \textbf{f)} hardware deployment. 


Each component can be customized as simple as entering specific parameters like wavelength for laser source, aperture size, approximation algorithms for diffraction modeling, detector design for measurement, selection of training algorithms, etc. In the rest of this section, we illustrate the programming capability of LightRidge by introducing the modules for each component of DONNs, including optical system setup, DONN construction, training, and deployment.} %To construct a simple feed-forward DONNs architecture, diffractive layers and detector can be stacked together and are fully differentiable. %To take advantages of Pytorch and existing machine learning algorithms, we design each module as differentiable and models can be trained easily with existing training engines for conventional neural networks, e.g., \texttt{Adam} for optimization.




\subsection{Global system definitions}  
\label{subsec:user_param}
%Unlike the compilation of conventional neural networks, the design, training, and deployment process of DONNs are highly sensitive to the physical optical setups, which are mostly determined by the application scenarios. 
DONN design and architecture are determined to the wavelength/frequency of the light that encodes the input features. {To initialize the compilation process of a DONN system w.r.t specific physical optical systems, the DONN architecture requires the following configurations supported by LightRidge -- (1) the laser profile such as wavelength/frequency and beam profile globally impacts the design, architecture exploration, and deployment of DONNs, (2) architecture configurations such as diffraction pixel size to be fabricated, number of diffraction units, DONNs depths, etc., need to carefully be configured for different ML tasks, (3) and the training and validation parameters of DONNs before and at the deployment stage. 

For example, as shown in Listing \ref{code:user_para}, depending on the laser source we have at hand, {the \texttt{wavelength} of the laser source will be set as 532nm, and the \texttt{laser profile} is set to be a Gaussian beam. Decided by the laser wavelength, we set the size of the diffraction unit in the layers (\texttt{unit\_size}) as 36$\text{um} \times$ 36um and the \texttt{distance} between source to diffractive layer, layers to layers, and layer to the detector is set to be 28cm}. The distance between each component can also be adjusted according to the requirements. %We are going to employ the proposed DONN system to realize the image classification with MNIST dataset (\texttt{dataset}). 
Training parameters are also initialized at this stage. As shown in this example, the training \texttt{Adam} optimizer \cite{kingma2014adam} implemented in PyTorch is set to be the optimizer with learning rate \texttt{lr} of 0.5. We will discuss how PyTorch optimizer can be leveraged directly to the DONN training process in Section \ref{subsec:phy_model}.}

%The parameters are provided for two parts -- (1) one for the customized optical system like wavelength for laser source and number of layers in the model; (2) the other one for the deep learning task with the DONN model like which dataset will be implemented and what optimization algorithm will be employed. For example, as shown in Listing \ref{code:user_para}, depending on the laser source we have at hand, {\color{red}the \texttt{wavelength} of the laser source will be set as 0.75mm, which lies in THz range, and the \texttt{laser profile} is set to be a Gaussian beam. Decided by the laser wavelength, we set the size of the diffraction unit in the layers (\texttt{unit\_size}) as 0.4$\text{mm} \times$ 0.4mm and the \texttt{distance} between source to diffractive layer, layers to layers, and layer to the detector is set to be 0.08m}. The distance between each component can also be adjusted according to the requirements. We are going to employ the proposed DONN system to realize the image classification with MNIST dataset (\texttt{dataset}). We set the \texttt{optimizer} as \texttt{Adam} with learning rate (\texttt{lr}) of 0.5. All the parameters proposed by users are taken into LightRidge to initialize the DONN model and its training.   

\begin{lstlisting}[language=Python, caption={Global definitions and system constraints of DONNs.}, label=code:user_para]
# define user parameters
# for laser source
lr.laser_profile.wavelength = 532e-9
lr.laser_profile.src_profile = 'Gaussian'
lr.laser_profile.waist = 2.9e-4
lr.laser_profile.aperture_radius = 2e-5
lr.laser_profile.aperture_dist = 2e-3
# for DONN systems
lr.diffraction.unit_size = 0.000036
lr.diffraction.distance = 0.28
lr.diffraction.sys_size = 200
depth = 5
lr.laser_profile.init()
lr.diffraction.init()
# for training
lr.model.train(optimizer = torch.optim.adam, lr = 0.5, batch_size = 500, epochs = 10)
\end{lstlisting}

\subsection{Laser profile} 
%\label{subsec:laser}
%With parameters provided and the python package LightRidge imported (import \texttt{lightRidge} as \texttt{lr}), components in an DONN model are ready to be customized. 
The first part of our framework is the design for the laser source in \texttt{lr.laser}, which will precisely offer conventional laser profiles that include laser specifications such as \texttt{wavelength}, \texttt{aperture}, etc. For example, we have implemented a widely used Gaussian beam profile taking the defined waist and two apertures, i.e., ring aperture and rectangle aperture, for applications. %For example, to implement a laser source with a Gaussian beam, we can call the block in the compiler by executing the single code \texttt{lr.laser.GaussBeam} and define its wavelength, aperture, and waist inside the block. 
Note that laser profile building block is critical to compiling any DONNs, since these parameters will be passed to all other building blocks discussed later. 

%Wavelength is a user-defined parameter for laser source. Currently, two apertures, ring aperture and rectangle aperture, are implemented in LightRidge. The profile for laser such as Gaussian profile can be implemented with \texttt{lr.laser.GaussBeam}. %With more characteristics of the laser source implemented in the simulation, users will get better consistency between numerical modeling and deployment.

\iffalse
\begin{lstlisting}[language=Python, caption= Customization of the laser source , label=code:laser_src]
import LightRidge as lr
# define laser source information
# aperture
aperture = RingAperture(radius, sys_size, aperture_dist, pixel_size=3.6e-5)
# profile
GaussMask = lr.laser.GaussBeam(waist=waist,size=size)
# input laser to the system
x_train = torch.square(torch.abs(
                    aperture(GaussMask(x_train)))
\end{lstlisting}
\fi

\subsection{Physics modelling of diffraction} 
\label{subsec:phy_model}

In the DONN system, phase modulations include trainable parameters, which realize data movements by light diffraction. %The input light wave and phase modulation will be both described with complex numbers. 
The main concept of DONNs in learning complex ML tasks is stacking such phase modulation and diffraction like conventional neural network layers, and optimize the phase parameters similarly as the conventional weight parameters. Thus, we introduce layer-wise physical modelling for diffraction and phase modulation with building block \texttt{lr.layers}. The algorithm for approximating the diffraction in the free-space system will be defined based on the laser source. Specifically, according to what we have discussed in Section \ref{subsec:diff_approx}, three major approximation algorithms in diffraction are implemented in our framework -- (1) \textit{Rayleigh-Sommerfeld Approximation}, implemented with Equation \ref{equ:sommerfeld}, which is the most accurate approximation algorithm but also a most complex one; (2) \textit{Fresnel Approximation}, implemented with Equation \ref{equ:fresnel}, which is an approximation for the propagation with parabolic wavefronts, namely the near field propagation; (3) \textit{Fraunhofer Approximation}, implemented with Equation \ref{equ:fraunhofer}, an approximation for the propagation with planar wavefronts, which is used to approximate the far field propagation \cite{tobin1997introduction}. Approximation algorithms can be selected by one of the following keywords, i.e., \texttt{Sommerfeld}, \texttt{Fresnel}, \texttt{Fraunhofer}, to the argument \texttt{approx} in the module \texttt{lr.layers.DiffractLayer}.
%Our system will take Rayleigh-Sommerfeld approximation as default.

The phase modulation encoded on the diffractive layers will be applied to the light wave by matrix multiplication as shown in Equation \ref{equ:phase_mod_matrix}. Specifically, when the input light wave projects on a diffractive layer, the input wave field is first transformed to Fourier domain by \textit{Fast Fourier Transform} (FFT) and matrix-multiplied with the {specific approximation functions selected} by the keyword \texttt{approx}. Then, the result matrix will be transformed to the time domain by \textit{inverse Fast Fourier Transforms} (iFFT) for phase modulation, where the matrix will be multiplied with another trainable matrix representing the phase changes.

The approximation functions are the most computation-intense cores in the compiler. Specifically, the forward function of diffraction requires FFT, iFFT, and complex matrix multiplications, which can take advantages of modern CPU and GPU platforms. {In addition, similarly to the front-end compilers of conventional neural networks, batched operations are critical in training, inference, and exploration runtime efficiency. Thus, LightRidge physics engine is designed to elaborate the conventional front-end ML compilers to improve runtime. Specifically, we develop the three diffraction approximations using PyTorch accelerated Fast Fourier Transforms modules. To enable batched operations on DONNs simulation, two-dimensional FFT and iFFT are deployed with batched complex tensors as inputs, which encode the input laser source or diffraction output from the previous layer. Complex matrix multiplications are mimicked with two parallel matrix multiplications. Unlike the state-of-the-art optics simulation framework LightPipe \cite{vdovin1997lightpipes}, the runtime of diffraction model simulation in LightRidge will natively support Intel’s MKL-FFT library \cite{wang2014intel} on Intel CPUs, and Nvidia’s cuFFT library \cite{podlozhnyuk2007fft} on CUDA devices, which have been carefully optimized in PyTorch. \textbf{Results in Section \ref{sec:runtime_result} show that our framework demonstrates up to 105$\times$ speedups on CPU, and up to 7,661$\times$ on CUDA devices, compared to LightPipe.} Detailed runtime comparisons are provided in Section \ref{sec:runtime_result}}.

%{\color{red}Additionally, to improve the accuracy performance of DONN systems with few diffractive layers ($\leq$ 3 layers), we introduce a hyperparameter \texttt{reg\_factor} in the simulation to regularize the gradients generated in the training process for DONN systems. The results in Section \ref{sec:evaluation} show our compiler with regularization will improve the simulation accuracy significantly for less complex DONNs. }
%For example, for the system with 1 diffractive layer, the simulation with LightRidge can get an accuracy of $0.98$ by setting the regularization factor as $90$ and it is $37\%$ increase compared to that in \cite{lin2018all} without regularization. For the system with 3 diffractive layers, the accuracy will increase from $0.91$ to $0.98$ with our compiler. 

\iffalse

\begin{lstlisting}[language=Python, caption=Example code blocks of diffractive layer modeling., label=code:phys_model]
import LightRidge as lr
# define the diffractive layer
lr.laser_profile.init()
lr.diffraction.init()
l1 = lr.layers.DiffractLayer(sys_size, pixel_size, approx='fresnel', ...)
l2 = lr.layers.DiffractLayer(sys_size, pixel_size, approx='fresnel', ...)
...
# Note: approx = 'sommerfeld' or 'fraunhofer' will select the other two approximation functions
\end{lstlisting}
\fi
%\cunxi{needs to show exact kernel implementation of all three approximations in PYTHON}

%\paragraph{\cunxi Kernel implementation basics}

%FFT IFFT Complex multiplication

%\paragraph{\cunxi Sommerfeld} h=?

%\paragraph{\cunxi Fresnel} h=?

%\paragraph{\cunxi Fraunhofer} h=?


%Another important component in the DONN system is the detector, which will capture the light intensity after diffraction and phase modulation. By analysing the intensity distribution on the detector with the pre-defined detector regions for different labels, we can get the final predication. LightRidge provides customization for detectors in \texttt{lr.layers.Detector}. Arbitrary observing pattern on detector plane can be designed with coordinates of the top-left corner of detector regions and the detector size provided. In our framework, the shape of each detector region is set to be square by default.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9 \linewidth]{isca2022-latex-template/figs/detector_api.pdf}
  \caption{Illustration example of the detector measurement enabled by \texttt{lr.layers.Detector} for a 10-class classification DONNs system. %, with the \texttt{x\_loc} and \texttt{y\_loc} arguments indicate the locations of the detector region for measuring the intensity for classification. %Note that activation function is only used for training the physical parameters in LightRidge, where physical measurement is performed directly with \texttt{argmax} on detector.
  }
 % \vspace{-3mm}
  \label{figs:detector}
\end{figure}

\subsection{Detector design}
 
{To convert the final outputs of DONNs into predictions (e.g., classification results), frequency-specific detectors are required to capture the intensity value of resulting light coming from the multi-layer diffraction and phase modulation. Specifically, by measuring the intensity distribution at the detector plane, carefully designed detector regions are important user-specific DONN architecture parameters. For example, for multi-label image classification tasks with $N$ classes, $N$ pre-defined detector regions will be specified that collect the intensity values of the light in each region, which is used for generating the final prediction using \texttt{argmax} just like conventional DNNs. %In other words, detector can be considered as the final layer for prediction in conventional neural networks. 
%Note that these pre-defined detector regions require domain-specific customization in different detectors and different laser profile. 
Thus, LightRidge provides customization for detectors via the compiler module \texttt{lr.layers.Detector}, which includes three major arguments: \textbf{(1)} 2D coordinates of the detector regions \texttt{x\_loc} and \texttt{y\_loc}, where the inputs are $N$ element lists, \textbf{(2)} detector size \texttt{det\_size}, which is the unit element in measuring the light intensity at the detector; \textbf{(3)} activation function used for training \texttt{activation}.} {We illustrate the Detector module in our framework using Figure \ref{figs:detector}, which construct a detector design for 10-class classification problem. %Note that the output of diffraction is in the complex-domain that contains both amplitude and phase information of the light, while the optical detector mostly measures the intensity of the light. Thus, to make final predictions in both emulation and experiments, the transformation from complex numbers to detectable intensity will be realized with the algorithm shown in Section \ref{sec:measure_pred}. During the training process, the light intensity over ten pre-defined detector regions, i.e., a $1 \times 10$ vector, read from the detector will first be applied with an activation function, which is \texttt{softmax} in this illustration, before \texttt{argmax} is applied for the final prediction. 
%While in the inference, \texttt{argmax} will be applied directly to the light intensity vector read from the detector, to incorporate with the physical optical detector that is very challenging to add nonlinearity.
}

\iffalse
\begin{lstlisting}[language=Python, caption={Detector design example in LightRidge.~Note that activation function is only used in training. Physical optical detector generates final prediction with \texttt{argmax}.}, label=code:det]
# Detector design, system size would be 200x200, ten classes in total, detector size would be 10x10
lr.layers.Detector(x_loc=[], y_loc=[], det_size, activation=torch.nn.functional.softmax, mode='intensity')
# mode = 'intensity' or 'amplitude' or 'phase' for analyzing other properties of the light output
\end{lstlisting}
\fi

 
\subsection{Diffractive neural architecture construction}

%With all components setup well, the DONN model will be simply constructed customized by setting a \texttt{class} model with all components imported. During model construction, LightRidge allows stacking arbitrary number of diffractive layers and placing layers at designed positions by adjusting the argument \texttt{distance}.

{As shown in Listing \ref{code:model_const}, with aforementioned fundamental optical modules, the DONN model can be simply constructed by stacking the diffractive layers modules implemented in \texttt{lr.layers}). Similar to conventional DNNs, the neural architecture of DONNs is a multi-layer feed-forward function consisting of a series of diffraction and phase modulation. Thus, to construct a DONNs model, LightRidge allows stacking arbitrary numbers of diffractive layers w.r.t designed physical optical system parameters, such as layer to layer distance, number of diffractive units, physical dimensions, per layer hardware parameters, etc. This DONNs \texttt{class} can be treated as a sequential container, where diffractive layer modules will be added to it in the order they are passed in and “chains” outputs to inputs sequentially for each subsequent module, finally returning the output of the last module.}

As a result, LightRidge compiler provides great flexibility for customizing the DONN model enabled by the versatile fundamental optical physics modeling. Here, we emphasize the following major versatile factors: 1) as discussed in Section \ref{sec:donn}, there is wide range of laser frequency that can be used; 2) heterogeneous design can be realized by defining different diffractive layers in the DONN system. Specifically, our compiler supports separate definitions for each diffractive layer. For example, the distance between the first and the second layer can be different from that between the second and the third layer by adjusting different \textit{distance} hyperparameters when implementing the second and the third layer.

\begin{lstlisting}[language=Python, caption=Model construction and CUDA acceleration of optical physics emulation examples., label=code:model_const]
###Model construction
# User-defined model composed based on components defined in 
# Physical Modelling and Detector Setup
class Model(torch.nn.Module):
    # initial arguments definition for the model
  def __init__(...)
        ...
    self.diffractive_layers_1=l1
    self.diffractive_layers_2=l2
        ...
    self.last_diffraction=layers.DiffractiveLayer(..., phase_mode = False)
    self.detector = lr.layers.Detector(...)
  def forward(self, x):
    x = self.diffractive_layers_1(x)
    x = self.diffractive_layers_2(x)
    ...
    x = self.last_diffraction(x)
    output = self.detector(x)
    return output

# emulation and training will be executed on Nvidia GPU.
model = Model(...).to("cuda")
\end{lstlisting}


\subsection{Training modules}

%{One of the critical components in LightRidge is to enable efficient physics-aware training of DONNs. For most of the conventional compilers for efficient hardware deployment, the compilation and optimizations are designed to enable efficient deployment of post-training models and automates optimization of low-level programs to hardware characteristics. Therefore, the training mechanisms of conventional neural networks are mostly supported by front-end ML compilers such as PyTorch, Tensorflow, etc. Note that training algorithms of conventional neural networks have been very well developed and can be easily extended and integrated in many other optimization tasks. For example, PyTorch optimizer module \texttt{torch.optim} implements various efficient optimization algorithms and has been highly optimized in performance and runtime. As most commonly used methods are already supported, and the interface is general enough, LightRidge training modules are built around the existing gradient descent optimization algorithms.}

%Most commonly used methods are already supported, and the interface is general enough, so that more sophisticated ones can be also easily integrated in the future.
 
%Then, machine learning task will be specified w.r.t the DONN model. For DONN model, the input information will be encoded on the laser beam. In optical domain, light will be described with complex numbers which involve real part and imaginary part. With the complex number description, we can get both amplitude and phase information of the information-carried light beam. In our framework, inputs will first be converted to complex domain by \texttt{lr.utils.data\_to\_cplex()}. At the output/detector plane, the intensity will be measured as the network output and compared with the ground truth label in the loss function, e.g., \texttt{MSELoss} for the loss function. With all components implemented as differentiable modules, the DONN model is fully differentiable, such that it can be trained with conventional automatic differentiation engine, e.g., \texttt{Adam} for optimization. 


Here, we introduce the training/optimization modules in LightRidge by focusing on ML tasks, particularly image classification problems, which natively supports PyTorch automatic differentiation (\texttt{autograd}) mechanism. For DONN model, the input information will be encoded on the laser beam. In optical domain, light will be described with complex numbers which involve real part and imaginary part. With the complex number description, we can get both amplitude and phase information of the information-carried light beam. In our framework, inputs will first be converted to complex domain by \texttt{lr.utils.data\_to\_cplex()}. At the output/detector plane, the intensity will be measured as the network output and compared with the ground truth label in the loss function, e.g., \texttt{MSELoss} for the loss function. With all components implemented as differentiable modules, the DONN model is fully differentiable, such that it can be trained with conventional automatic differentiation engine, e.g., \texttt{Adam} for optimization. 

As a result, in the forward function, the DONNs model makes its prediction based on the diffraction propagation and the prediction of the given feature is then made at the detector plane. In other words, it runs the input data through every diffraction and phase modulation to make its prediction. During the backpropagation phase, the DONNs will adjust its \textbf{phase modulation parameters} proportionate to the error made in the forward function. Note that the phase modulation parameters correspond to specific physical parameters (e.g., thickness of materials) or supplying voltage value on devices (e.g., SLMs and phase change material). Similarly, this is done by traversing backward from the output, collecting the derivatives of the error with respect to the parameters of diffraction functions (i.e., FFT, IFFT, and complex-domain matrix multiplication), and optimizing the parameters using gradient descent algorithms.


\iffalse

\begin{lstlisting}[language=Python, caption=Model training. The inputs will first be converted to complex domain. Conventional optimization engines can be employed in the training., label=code:training]
# Training/ Testing setup
# Convert original gray-scale images into complex domain
x_train, y_train = lr.utils.data_to_cplex(train_loader)
x_test, y_test = lr.utils.data_to_cplex(test_loader)
# Apply laser mask to input images
x_train = torch.square(torch.abs(aperture(GaussMask(x_train)))
# Define loss criterion, optimization algorithm, etc. 
def train():
  ...
  optimizer = torch.optim.Adam(model.parameters(), lr=lr)
  criterion = torch.nn.MSELoss(reduction='sum')
  train_loss_ = criterion(train_outputs, train_labels)
\end{lstlisting}

\fi


\iffalse
\begin{lstlisting}[language=Python, caption=Back-end deployment support and propagation measurement., label=code:model_backend]
# simulation visualization
# view phase modulation
model.phase_view()
# view propagation 
model.prop_view()
# Generate phase mask with 3D printer
model.to_3d_render(3d_print_specs)
# Generate phase mask with SLM
model.to_slm(slm_specs)
\end{lstlisting}
\fi

%The code in our system is designed based on \texttt{pytorch}. Taking advantage of GPU and \texttt{pytorch}, we modulate the design components, simplifying the process of designing diffractive optical neural network. With our system, users can simulate their designed diffractive models easily and the design efficiency can be improved greatly.


\subsection{Complex-domain Regularization}
\label{sec:regu}

In our implementation, considering the physics in optics, the DONN system is described and emulated with complex numbers. According to \cite{lin2018all} and Equation \ref{equ:phase_mod_matrix}, the training for DONN system is more phase modulation dominated and the intensity at the end of diffraction will decrease exponentially as the number of diffractive layers increases, which means a regularization between amplitude and phase is required to avoid gradient vanishing and explosion in training process. Thus, we introduce a novel regularization factor $\lambda$ in the forward function described in {Equation \ref{equ:phase_mod_matrix}} to improve the training efficiency, which can flexibly change the gradient scales between amplitude and phase modulations. Specifically, $\lambda$ is applied to amplitude vector $A$ in Equation \ref{equ:phase_euler}. 
%Let $\mathcal{M}$ as the mapping of $(w^{i, j}, A, P) \xrightarrow{\mathcal{M}} w^{i,j}_{\mathbb{C}}$. Let $\nabla w^{i,j}_{\mathbb{C}}$ be the upstream gradient to calculate $\nabla w^{i,j}$. The difference of the gradient updates can be summarized as follows: 
\iffalse
\begin{equation*}
\begin{split}
   \nabla w^{i,j} = {\nabla w^{i,j}_{\mathbb{C}}} \cdot \frac{ \frac{\partial \mathcal{M}}{\partial{w^{i, j}}} \cdot A + \frac{\partial \mathcal{M}}{{\partial{w^{i, j}}}} \cdot P}{2} ~~~~ \xRightarrow{~~~~\lambda~~~~} ~~~~ \\
   \nabla w^{i,j}_{reg} = \nabla w^{i,j}_{\mathbb{C}} \cdot \frac{ \frac{1}{\lambda} \cdot ( {\frac{\partial{\mathcal{M}}}{\partial{w^{i, j}}} \cdot {A}}) + \frac{\partial{\mathcal{M}}}{\partial{w_{i, j}}} \cdot P}{2}
\end{split}
    \label{equ:grad}
\end{equation*}
\fi
%The gradients will be backpropagated as shown in Equation \ref{equ:grad}. 
%Since in DONNs system, the intensity of the input light decreases exponentially as the diffractive layers increase, the amplitude used in our system will decrease exponentially as expected. For the two integrated parameters, phase and amplitude, controlled by one device discrete state, amplitude will change with the depth implemented in the system while phase will not. Thus, the regularization factor $\lambda$ is introduced to avoid gradient explosion and vanishing, which compensates the effects caused by the change of system depth. According to Equations \ref{equ:grad}, this regularization factor adjusts the weight of upstream gradients calculated on the amplitude and phase. 

Since in DONN system, the intensity of the input light decreases exponentially as diffractive layers increase, the weight of amplitude modulation in forward and backward propagation are expected to decrease exponentially, as the number of layers increases. Thus, the optimal value for the algorithmic parameter $\lambda$ needs to be explored for different DONNs architectures. Empirically, $\lambda$ should be $\geq$1, i.e., compensating the loss for the intensity after propagating through each diffractive layer. %In Section \ref{subsec:conf_test}, we explore the performance of the proposed regularization technique with 1, 3 and 5 diffractive layers in DONNs, which confirms the discussed regularization characteristic.
%Moreover, as the results in section \ref{sec:result_regu} show, even though systems with different diffractive layers can all be trained to acquire a decent accuracy performance with no much difference by adjusting the regularization factor in training process, the classification confidence can vary significantly. As diffractive layers increase in the system, the classification problem can be finely tuned and explored with more neurons involved. Thus, the predictions will be more confident. 

\subsection{Hardware deployment and visualization}
Users can view the phase modulation for each diffractive layer by executing \texttt{model.phase\_view} and view the propagation process by executing \texttt{model.prop\_view}. More importantly, the proposed compiler directly supports various popular hardware deployment w.r.t to specific laser source. Specifically, LightRidge supports different fabrication/deployment methods, e.g., SLMs for laser in visible range and 3D printed phase mask for THz systems. Our framework can directly interface with these two types of hardware backends, e.g., \texttt{model.to\_slm} for EXULUS-HD1 SLMs and \texttt{model.to\_3d\_render} for FormLab 3D printers.
